Bandwidth Utilization Side-Channel on ML Inference Accelerators

Accelerators used for machine learning (ML) inference provide great performance benefits over CPUs. Securing confidential model in inference against off-chip side-channel attacks is critical in harnessing the performance advantage in practice. Data and memory address encryption has been recently proposed to defend against off-chip attacks. In this paper, we demonstrate that bandwidth utilization on the interface between accelerators and the weight storage can serve a side-channel for leaking confidential ML model architecture. This side channel is independent of the type of interface, leaks even in the presence of data and memory address encryption and can be monitored through performance counters or through bus contention from an on-chip unprivileged process.

==> default.tex <==
\begin{comment}


\section{Introduction}

This document provides instructions for submitting papers to ISCA
2021.  In an effort to respect the efforts of reviewers and in the
interest of fairness to all prospective authors, we request that all
submissions to ISCA 2021 follow the formatting and submission rules
detailed below. Submissions that violate these instructions may not be
reviewed, at the discretion of the program chair, in order to
maintain a review process that is fair to all potential authors. This
document is itself formatted using the ISCA 2021 submission format. The
content of this document mirrors that of the submission instructions
that appear on the conference website. All questions regarding paper
formatting and submission should be directed to the program chair.

\subsection{Format Highlights}

Here are the format highlights in a nutshell:
\begin{itemize}
\item Paper must be submitted in printable PDF format.
\item Text must be in a minimum 10pt Times font, see Table~\ref{table:formatting}.
\item Papers must be at most 11 pages (not including references) in a
  two-column format.
\item No page limit for references.
\item Each reference must specify {\em all} authors, i.e., no {\em et al.}
\end{itemize}

\subsection{Paper Evaluation Objectives} 
The committee will make every effort to judge each submitted paper on
its own merits. There will be no target acceptance rate. We expect to
accept a wide range of papers with appropriate expectations for
evaluation --- while papers that build on significant past work with
strong evaluations are valuable, papers that open new areas with less
rigorous evaluation are equally welcome and especially encouraged. We
also acknowledge the wide range of evaluation methodologies in ISCA including
modeling, simulation, prototyping, experimental implementation, real
product evaluation, etc. 


    


\subsection{Paper Formatting}
Papers must be submitted in printable PDF format and should contain a
{\em maximum of 11 pages} of single-spaced two-column text, {\bf not
  including references}.  You may include any number of pages for
references, but see below for more instructions.  If you are using
\LaTeX~\cite{lamport94} to typeset your paper, then we suggest that
you use the template used to prepare this document, which you can find
on the ISCA 2021 website. If you use a different
software package to typeset your paper, then please adhere to the
guidelines given in Table~\ref{table:formatting}.  

\begin{scriptsize}
\begin{table}[h!]
  \centering
  \caption{Formatting guidelines for submission.}
  \label{table:formatting}
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Field} & \textbf{Value}\\
    \hline
    \hline
    File format & PDF \\
    \hline
    Page limit & 11 pages, {\bf not including}\\
               & {\bf references}\\
    \hline
    Paper size & US Letter 8.5in $\times$ 11in\\
    \hline
    Top margin & 1in\\
    \hline
    Bottom margin & 1in\\
    \hline
    Left margin & 0.75in\\
    \hline
    Right margin & 0.75in\\
    \hline
    Body & 2-column, single-spaced\\
    \hline
    Space between columns & 0.25in\\
    \hline
    Line spacing (leading) & 11pt \\
    \hline
    Body font & 10pt, Times\\
    \hline
    Abstract font & 10pt, Times\\
    \hline
    Section heading font & 12pt, bold\\
    \hline
    Subsection heading font & 10pt, bold\\
    \hline
    Caption font & 9pt (minimum), bold\\
    \hline
    References & 8pt, no page limit, list \\
               & all authors' names\\
    \hline
  \end{tabular}
\end{table}
\end{scriptsize}

{\em Please ensure that you include page numbers with your
  submission}. This makes it easier for the reviewers to refer to
different parts of your paper when they provide comments. Please
ensure that your submission has a banner at the top of the title page,
similar to this document, which contains the submission number and the
notice of confidentiality.  If using the template, just replace `NaN'
with your submission number. 

\subsection{Content}
Reviewing will be {\em double blind} (no author list); therefore,
please do not include any author names on any submitted documents
except in the space provided on the submission form.  You must also
ensure that the metadata included in the PDF does not give away the
authors. If you are improving upon your prior work, refer to your
prior work in the third person and include a full citation for the
work in the bibliography.  For example, if you are building on {\em
  your own} prior work in the
papers~\cite{nicepaper1,nicepaper2,nicepaper3}, you would say
something like: "While the authors of~\cite{nicepaper1,nicepaper2,nicepaper3} did X,
Y, and Z, this paper additionally does W, and is therefore much
better."  Do NOT omit or anonymize references for blind review.  There
is one exception to this for your own prior work that appeared in IEEE
CAL, arXiv, workshops without archived proceedings, etc.\ as
discussed later in this document. 

\noindent\textbf{Figures and Tables:} Ensure that the figures and
tables are legible.  Please also ensure that you refer to your figures
in the main text.  Many reviewers print the papers in
gray-scale. Therefore, if you use colors for your figures, ensure that
the different colors are highly distinguishable in gray-scale. 

\noindent\textbf{References:}  There is no length limit for
references. {\em Each reference must explicitly list all authors of
  the paper.  Papers not meeting this requirement will be rejected.}
Since there is no length limit for the number of pages
used for references, there is no need to save space here. 


\section{Paper Submission Instructions}

\subsection{Guidelines for Determining Authorship}
IEEE guidelines dictate that authorship should be based on a {\em
  substantial intellectual contribution}. It is assumed that all
authors have had a significant role in the creation of an article that
bears their names. In particular, the authorship credit must be
reserved only for individuals who have met each of the following
conditions: 

\begin{enumerate}
\item Made a significant intellectual contribution to the theoretical
  development, system or experimental design, prototype development,
  and/or the analysis and interpretation of data associated with the
  work contained in the article; 

\item Contributed to drafting the article or reviewing and/or revising
  it for intellectual content; and 

\item Approved the final version of the article as accepted for publication, including references.
\end{enumerate}

A detailed description of the IEEE authorship guidelines and
responsibilities is available online.\footnote{\url{https://www.ieee.org/publications_standards/publications/rights/Section821.html}} Per
these guidelines, it is not acceptable to award {\em honorary}
authorship or {\em gift} authorship. Please keep these guidelines in
mind while determining the author list of your paper. 

\subsection{Declaring Authors}
Declare all the authors of the paper upfront. Addition/removal of
authors once the paper is accepted will have to be approved by the
program chair, since it potentially undermines the goal of eliminating
conflicts for reviewer assignment. 

\subsection{Areas and Topics}
Authors should indicate specific topics covered by the paper on the
submission page. If you are unsure whether your paper falls within the
scope of ISCA, please check with the program chair --- ISCA is a broad,
multidisciplinary conference and encourages new topics. 

\subsection{Declaring Conflicts of Interest}

Authors must register all their conflicts on the paper submission
site. Conflicts are needed to ensure appropriate assignment of
reviewers. If a paper is found to have an undeclared conflict that
causes a problem OR if a paper is found to declare false conflicts in
order to abuse or `game' the review system, the paper may be rejected. 

Please declare a conflict of interest with the following people for any author of your paper.
A conflict occurs in the following cases:
\begin{enumerate}
\item Between advisor and advisee forever. 
\item Between family members forever. 
\item Between people who have collaborated in the last 5 years. This
  collaboration can consist of a joint research or development
  project, a joint paper, or when there is direct funding from the
  potential reviewer (as opposed to company funding) to an author of
  the paper. Co-participation in professional activities, such as
  tutorials or studies, is not cause for conflict. When in doubt, the
  author should check with the Program Chair. 
\item Between people from same institution or who were in the same
  institution in the last 5 years.  
\item Between people whose relationship prevents the reviewer from
  being objective in his/her assessment. 
\end{enumerate}

`Service' collaborations, such as co-authoring a report for a
professional organization, serving on a program committee, or
co-presenting tutorials, do not themselves create a conflict of
interest. Co-authoring a paper that is a compendium of various
projects with no true collaboration among the projects does not
constitute a conflict among the authors of the different projects. On
the other hand, there may be others not covered by the above with whom
you believe a COI exists, for example, an ongoing collaboration which
has not yet resulted in the creation of a paper or proposal. Please
report such COIs; however, you may be asked to justify them. Please be
reasonable. For example, you cannot declare a COI with a reviewer just
because that reviewer works on topics similar to or related to those
in your paper.  The program chair may contact co-authors to explain a COI
whose origin is unclear. 

Most reviews will be solicited among the members of the PC and the ERC, but other
members from the community may also write reviews. Please declare all
your conflicts (not just restricted to the PC and ERC) on the
submission form. When in doubt, contact the program chair. 


\subsection{Concurrent Submissions and Workshops}
By submitting a manuscript to ISCA 2021, the authors guarantee that
the manuscript has not been previously published or accepted for
publication in a substantially similar form in any conference,
journal, or the archived proceedings of a workshop (e.g., in the
ACM/IEEE digital libraries) --- see exceptions below. The authors also
guarantee that no paper that contains significant overlap with the
contributions of the submitted paper will be under review for any
other conference or journal or an archived proceedings of a workshop
during the ISCA 2021 review period. Violation of any of these
conditions will lead to rejection. 

The only exceptions to the above rules are for the authors' own papers
in (1) workshops without archived proceedings such as in the ACM/IEEE
digital libraries (or where the authors chose not to have their paper
appear in the archived proceedings), or (2) venues such as IEEE CAL or
arXiv where there is an explicit policy that such publication does not
preclude longer conference submissions.  In all such cases, the
submitted manuscript may ignore the above work to preserve author
anonymity. This information must, however, be provided on the
submission form --- the program chair will make this information available
to reviewers if it becomes necessary to ensure a fair review.  
If you have already put your manuscript on arXiv, in the interest of 
double blind review, modify the title for the version you submit to ISCA.
As always, if you are in doubt, it is best to contact program chairs. 


Finally, the ACM/IEEE Plagiarism Policies\footnote{\url{http://www.acm.org/publications/policies/plagiarism_policy}\\
\url{https://www.ieee.org/publications_standards/publications/rights/plagiarism_FAQ.html}}
cover a range of ethical issues concerning the misrepresentation of
other works or one's own work. 
\end{comment}

==> threatModel.tex <==
\section{Threat model}
\label{sec:ThreatModel}

The ML inference execution should be protected from malicious cloud hypervisor or system software outside of the accelerator. Data confidentiality and data access pattern for both model vendor and user should be ensured in memory (DRAM or LLC). Moreover, the cloud hypervisor can monitor accelerator memory bandwidth for quality-of-service (QoS) and traffic management. A malicious traffic management software can use this utilization information to infer dimensions of model layers.
The confidential execution should be isolated from other tenants in the form of co-executing inference services on the same accelerator or time-shared distrustful models. This includes \textbf{(1)} Buffer overflow attacks of on-chip storage like scratchpad and on control/data queues holding secret data; \textbf{(2)} Queue contention attacks; \textbf{(3)} Scratchpad/data buffer use-after-free attacks; \textbf{(4)} Compute execution time variations.



\begin{comment}


\system{} is designed to safeguard security properties \textbf{(P1-P4)} under all deployment settings against {\em on-chip} attackers.
In this section, we first discuss the threat models that \system{} concerns and
then present our analysis of attack surfaces in ML accelerator inference execution.

% Figure~\ref{fig:VulAnal} demonstrates the attack surfaces in 
% Defence mechanisms for 1-4 (greyed) are studied vividly in prior works while \system{} guarantees the remaining vulnerability mitigation.
\subsection{Threat model}
We assume a strong adversary including cloud hypervisor,
privileged and unprivileged software running in cloud snooping/contending both on-chip and off-chip resources.
Malicious privileged software can access secret data from memory and snoop memory-accelerator bus with high-resolution timers.
Other tenants can contend for memory read/write bus with victim execution.
Moreover, hypervisor and tenants can observe and contend for on-chip resources
including scratchpad, execution units and control victim execution through dependency queues between load, compute and store blocks.
\end{comment}

==> vulnerability.tex <==
\section{Vulnerability analysis}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/threat_model_vul2.pdf}
    \caption{\textbf{MLaaS accelerator vulnerabilities with various attack categories. Black circles are handled by \system{} while greyed circles are handled by baseline secure platform. }}
    \label{fig:VulAnal}
\end{figure}


The vulnerabilities arise for a cloud ML accelerator inference is shown in Figure~\ref{fig:VulAnal}.

\begin {enumerate}[leftmargin=*,label=(\alph*)]
    \itemsep0em
    \item The platform and the remote tenants (model service provider and user) must create a secure channel like TLS to communicate sensitive information to eliminate eavesdropping and man-in-the-middle attacks (\circled{1}).
    \item Remote attestation of the cloud platform ensuring: 
    \begin{itemize}
        \item Accelerator hardware is provided by a trusted manufacturer.
        \item Accelerator driver runs in an isolated environment preventing side-channel leakage \circled{2} and data confidentiality violations \circled{3} from the OS, hypervisor and other privileged/non-privileged software on both the CPU and main memory. 
        \item The ML compiler framework and driver are sourced from a trusted software provider.
    \end{itemize}
    \item Key management systems that handle cryptographic keys to either set up communication channels or provision memory encryption for the accelerator are in the trusted code base.
    \item Physical access on memory to impact memory integrity or snoop secrets from the address bus, this platform can protect with relevant defenses \cite{MorphCount, Vault, mee, aegis, bonsai-merkle-tree, Phantom, PathORM} by extending the memory controller \circled{4}. 
    \item Private data and/or model should be encrypted 
     
\end{enumerate}


\begin{comment}


\begin {enumerate}[leftmargin=*,label=(\alph*)]
    \itemsep0em
\item The host platform and the remote tenants (model service provider and user) create a secure channel like TLS to communicate sensitive information to eliminate eavesdropping and man-in-the-middle attacks (\circled{1} in Figure~\ref{fig:VulAnal}).
\item The cloud instance provides an attestation service to assure the clients that
\begin{itemize}
    \itemsep0em
\item All hardware on the platform is provided by a trusted manufacturer. The platform is free from any hardware trojans in our prototype with accelerator bitstream hash checked during secure boot.
\item The accelerator driver run in an trusted execution environment (like SGX, trustzone). The ability to isolate the driver prevents side-channel leakage \circled{2} and data confidentiality violations \circled{3}  from the OS, hypervisor and other privileged/non-privileged software on both the CPU and main memory. 
\item The ML compiler framework and driver are sourced from a trusted software provider and can be deployed to run in a TEE.
\end{itemize}
Attestation protocols remain same whether a `secure processor' implements a RISC CPU (like Aegis ~\cite{aegis} or Sanctum~\cite{Sanctum}) or an application-specific accelerator logic. Attestation enables platform authentication (whose identity is vouched for by a public-key certificate authority) on which the user can execute a workload.

%\item Confidential data stored in main memory can be protected using encryption \cite{AMD-SME,AWS-Graviton2,Intel-TME}.
\item Any key management systems that handle cryptographic keys to either set up communication channels or provision memory encryption for the accelerator are in the trusted code base.

\item For deployment scenarios where the attacker has physical access to the memory to impact memory integrity or snoop secrets from the address bus, this platform can protect with relevant defenses \cite{MorphCount, Vault, mee, aegis, bonsai-merkle-tree, Phantom, PathORM} 
% or address-buses 
by extending the memory controller \circled{4}. 

\ignore {Sensitive data stored in main memory can be protected using encryption and its integrity can be verified on every access.While  a  simple  implementation  of  integrity  verification can  be  performance  intensive,  recent  work  has  shown  this overhead can be significantly reduced [28], [30], [34]
% The \system{} prototype excludes these vulnerabilities as
Many recent commercial products include encrypted DRAM \cite{AMD-SME,AWS-Graviton2,Intel-TME} without integrity protection ~\cite{MorphCount,mee,aegis,bonsai-merkle-tree} or
address bus protection \cite{MorphCount, Vault, Phantom, PathORM}  in cloud deployments. 
}
\end{enumerate}



\subsection{Vulnerabilities handled by \system{} }
\label{sec:VulAnal}
%Vulnerabilities 13 and 14 are outside the scope of our threat model. In Table~\ref{tab:VulAnal} we highlight some defenses proposed by prior art. In section \ref{sec:implement} we see how these defenses can be easily composed with a \system{} platform.
 

%\begin{itemize}[leftmargin=*]

\subsubsection{Secret data encryption} Private data and/or model present in DRAM should be encrypted to prevent data confidentiality breach from cloud software \circled{5}.
\subsubsection{Memory bandwidth snooping}
\label{subsec:mem_bw_attack}
Modern chips commonly include high precision memory bandwidth performance counters for performance debugging purposes. These may also be used by a cloud provider for ensuring quality of service (QoS) across multiple tenants using the same platform. However these performance counters can end up creating a utilization side channel \circled{6} at the memory bus interface. Figure~\ref{fig:vgg16_end2end} shows the memory traffic of all the convolution layers of VGG16. Each of the layers utilizes different amounts of memory bandwidth based on tile size. 
Figure \ref{fig:vgg16_layer5} zooms in on layer 5 which consists of 32 tiles. The read bandwidth trace leaks the number of tiles due bandwidth variations at tile boundaries.The kernel size can be reverse engineered from the bandwidth consumption. In Section~\ref{sec:evaluate_security}, we demonstrate that a classifier can detect layer boundaries and layer types based on change in traffic shape and bandwidth. Upon successful leakage of the structure of the model, the attacker can craft custom inputs and devise an attack to determine the weights\cite{scnn, ReverseCNN}.  Interestingly, this attack can be effected solely by observing bandwidth variations using performance counters even when the data and address buses are protected. To the best of our knowledge, our work is the first to make this observation and design
%This attack works even on encrypted/authenticated data for both spatial and temporal sharing with private models. Public model with private inputs are not susceptible to this attack as dynamic zero pruning is disabled on private data outputs and the input shape is known for private input threat model.  
% \system{} is resilient to this attack by obfuscating RAW dependencies and model bandwidth variations with the memory traffic shaper discussed in section~\ref{subsec:traffic-shaper}.
\system{} to defend against such \textit{observation channel} attacks (Section~\ref{subsec:traffic-shaper}).

\subsubsection{Shared memory controller} A malicious tenant can stall or control the execution time of a victim by creating a contention on the load/store queue in a shared memory controller \circled{7}. \system{} prevents such attacks by providing separate load/store queues for each tenant with the bandwidth requirement declaration upfront as model definition. 
\subsubsection{Shared instruction queues}
Shared instruction queues allow the attacker to perform cyclic attacks like prime-and-probe \circled{8} by inserting instructions between victim execution and creating a covert channel to leak data. \system{} design closes this vulnerability with private instruction queues. (Section~\ref{subsec:scheduler-instruction-queue}).

\subsubsection{Shared dependency queues}
The load, compute, and store units of the accelerator are controlled through dependency queues.
An attacker can corrupt control dependencies of the victim program -- e.g., by triggering execution units before data loading -- and violate read-after-write (RAW) dependencies \circled{9} . 
\system{} addresses this through partitioned dependency queues for each tenant (Section~\ref{subsubsec:partitionDependencyQueue}).
% The \system{} microarchitecture partitions these dependency queues to restrict malicious tenants from observing or tampering with other tenants. 
%The \system{} driver allocates sufficient number of queue entries to each tenant (determined using auto-tuning) to remove queue contention.


\subsubsection{Shared access to scratchpads} ML accelerators typically use scratchpads instead of a cache hierarchy as these provides explicit control on data allocation and enable software to optimize memory utilization. This also rids us of cache timing based side-channels. However, shared access to the scratchpad can help an attacker read out stale secrets belonging to the victim by computing on a scratchpad region without loading any data after a victim's execution \circled{10}.
\system{} uses partitioned scratchpads, private data zeroization logic, and instruction base/bound check
to address this threat
(Section~\ref{subsubsec:scratchpad}).


% has private instruction queues for each tenant to ensure that tenants do not infer secrets via contention for the queue.

\subsubsection{Shared access to execution units}
Sharing of execution units can lead to cross-tenant contention attacks in a multi-tenant accelerator \circled{11}. \system{} schedules execution units among different tenants based on their program phases. 
%\end{itemize}
\quad

\subsubsection{Variable time GEMM/ALU unit}
Since ML weights are typically sparse, data driven optimizations leading to execution time variability leaking sensitive model/input data during spatial sharing. \system{} 
generates constant time execution instructions on private data operations.
% (Section~\ref{subsec:constantEU}).
%compiler performs dataflow analysis to identify private inputs and local variables and 

% \sarbartha{New figure with read channel info 1(a) update}



\begin{figure}[hbtp]
    \centering
    \begin{subfigure}{\linewidth}
        \centerline{\includegraphics[width=\linewidth]{Figures/vgg16_end2end_real_traffic.pdf}}
        \subcaption{\label{fig:vgg16_end2end}\textbf{Memory bandwidth of layers in vgg16.}}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centerline{\includegraphics[width=\linewidth]{Figures/vgg16_layer5_real_traffic.pdf}}
        \subcaption{\label{fig:vgg16_layer5}\textbf{Read bandwidth of the 5th layer in vgg16.}}
    \end{subfigure}
    \caption{\label{fig:vgg16_attack_demo}\textbf{Different layers in vgg16 network utilizes different memory bandwidth, while bursts within each layer show number of tiles.}
    }
\end{figure}


%\system{} driver and compiler passes can be run in an isolated environment like Intel SGX or ARM Trustzone.
\subsection{Out of Scope}
\system{} focuses on defending against on-chip attackers.
Physical attacks to accelerator and memory in data center is out of scope. 
Similarly, analog side channels like electromagnetic radiations, power and temperature variations require physical access, thus are out of scope of \system{}.
In practice, deployments on physically guarded data-centers are a common way to address physical access attacks without integrity/ORAM checks -- e.g., AWS, Google cloud, and Azure will sign business associate agreements that guarantee physical security.
In addition,
Denial-of-Service (DoS) attacks by an attacker on the network connection between the remote client and the accelerator driver and termination of accelerator driver is out-of-scope.
% Moreover, accelerator driver can be susceptible to TEE side-channels\cite{Foreshadow} and is out-of-scope.




For \system{} prototype on an FPGA, we trust device manufacturer(Xilinx) and associated software(Vivado suite) to generate bitstream equivalence to our design. The FPGA bitstream hash is checked during co-processor secure boot and is assumed free of hardware trojans. Dynamic reprogramming is disabled in our setup to prevent runtime introduction of hardware trojans.
% But the bitstream is assumed to be free of hardware trojans.

    
\end{comment}
